Quantization Aware Training, ERNIE and Kurtosis Regularizer: a short empirical study

Pre-trained language models like Ernie or Bert are currently used in many applications. These models come with a set of pre-trained weights typically obtained in unsupervised/self-supervised modality on a huge amount of data. After that, they are fine-tuned on a specific task. Applications then use these models for inference, and often some additional constraints apply, like low power-budget or low latency between input and output. The main avenue to meet these additional requirements for the inference settings, is to use low precision computation (e.g. INT8 rather than FP32), but this comes with a cost of deteriorating the functional performance (e.g. accuracy) of the model. Some approaches have been developed to tackle the problem and go beyond the limitations of the PTO (Post-Training Quantization), more specifically the QAT (Quantization Aware Training, see [4]) is a procedure that interferes with the training process in order to make it affected (or simply disturbed) by the quantization phase during the training itself. Besides QAT, recently Intel-Habana Labs have proposed an additional and more direct way to make the training results more robust to subsequent quantization which uses a regularizer, therefore changing the loss function that drives the training procedure. But their proposal does not work out-of-the-box for pre-trained models like Ernie, for example. In this short paper we show why this is not happening (for the Ernie case) and we propose a very basic way to deal with it, sharing as well some initial results (increase in final INT8 accuracy) that might be of interest to practitioners willing to use Ernie in their applications, in low precision regime.

==> Kurtosis paper/buffer.tex <==



On this line of thinking, to see why it would be worth having high level entities like numerosity directly accessible and controllable in a generative process, we can consider an intelligent agent tasked to plan a series of actions to reach a predefined goal: for this agent, the possibility to generate hypothesis and simulate the effect of choices it is a key capability for planning; in this scenario, generative models may bring the necessary tools to generate hypothesis, and the possibility to have this generation process controlled by specific high-level qualities (like numerosity) is key to the interpretability of the actions of the agent.

, \textbf{TODO:check if this could be extended to no labels, forcing only the IS-score like cost function only and then make JS on the output of the classifier. It should be possible just changing the class loss on real to the same expression i use for the IS-Score like cost on fake, which is what is done in CatGAN to be unsupervised and use only the number of classed and not labels } 

\begin{enumerate}
  \item the images from the dataset used as described above, on the first "generative" line 
  \item the labels of the images encoded as distributed pattern of activity of the output neurons of the second "generative" line. For this pourpose the output layer of this second generative line was modeled as softmax to approximate a one-hot representation of the labels.
\end{enumerate}

The statement deserves a clarification: the input image should be thought as a vector respresented in a space whose dimensionality depends on the representation used; finding a representation of the input that is totally or partially semantically disentangled means that such representation uses a set, or a subset, of axis that are orthogonal among them, and along which we can quantify properties that we recognize as semantically meaningful and along which we can quantify properties that we recognize as semantically meaningful and independent among them. As we will see, learning high level concepts from the statistic of the input (e.g. dataset of images) may not be a straightforward task even for the InfoGAN model, as it was for MNIST, since the semantically meaningful variations of "higher level of abstraction" can be overhelmed by other statistical variations in the data connected to much lower level features, like purely graphical for example, that must be somehow ignored by the learning process in order to let emerge the variations that are carrying the semantic relevant information we are hoping to learn. It seems to be the way the learning process is driven that will leave the higher level semantical features to emerge. Clearly the relevance of this point is strictly connected the kind of semantical dimension we want to isolate.}


The subitizing sense is considered to be an innate cognitive function of humans and primates that enables them to precisely evaluate and respond to visual stimuli even in the absence of the development of any abstract cognitive skills, whereas the ANS is indeed an approximate number system for which experimental data show that is characterized by a constant coefficient of variation (CV: the ratio between the standard deviation and the absolute value of the mean of the estimations provided by the subject under test), and which typically get better with experience.

   \begin{gather}
     a=b \label{one} \\
     c=d \label{two} \\
     e=f \label{three}
   \end{gather}
   \eqref{one} \eqref{two} \eqref{three}

==> buffer.tex <==



On this line of thinking, to see why it would be worth having high level entities like numerosity directly accessible and controllable in a generative process, we can consider an intelligent agent tasked to plan a series of actions to reach a predefined goal: for this agent, the possibility to generate hypothesis and simulate the effect of choices it is a key capability for planning; in this scenario, generative models may bring the necessary tools to generate hypothesis, and the possibility to have this generation process controlled by specific high-level qualities (like numerosity) is key to the interpretability of the actions of the agent.

, \textbf{TODO:check if this could be extended to no labels, forcing only the IS-score like cost function only and then make JS on the output of the classifier. It should be possible just changing the class loss on real to the same expression i use for the IS-Score like cost on fake, which is what is done in CatGAN to be unsupervised and use only the number of classed and not labels } 

\begin{enumerate}
  \item the images from the dataset used as described above, on the first "generative" line 
  \item the labels of the images encoded as distributed pattern of activity of the output neurons of the second "generative" line. For this pourpose the output layer of this second generative line was modeled as softmax to approximate a one-hot representation of the labels.
\end{enumerate}

The statement deserves a clarification: the input image should be thought as a vector respresented in a space whose dimensionality depends on the representation used; finding a representation of the input that is totally or partially semantically disentangled means that such representation uses a set, or a subset, of axis that are orthogonal among them, and along which we can quantify properties that we recognize as semantically meaningful and along which we can quantify properties that we recognize as semantically meaningful and independent among them. As we will see, learning high level concepts from the statistic of the input (e.g. dataset of images) may not be a straightforward task even for the InfoGAN model, as it was for MNIST, since the semantically meaningful variations of "higher level of abstraction" can be overhelmed by other statistical variations in the data connected to much lower level features, like purely graphical for example, that must be somehow ignored by the learning process in order to let emerge the variations that are carrying the semantic relevant information we are hoping to learn. It seems to be the way the learning process is driven that will leave the higher level semantical features to emerge. Clearly the relevance of this point is strictly connected the kind of semantical dimension we want to isolate.}


The subitizing sense is considered to be an innate cognitive function of humans and primates that enables them to precisely evaluate and respond to visual stimuli even in the absence of the development of any abstract cognitive skills, whereas the ANS is indeed an approximate number system for which experimental data show that is characterized by a constant coefficient of variation (CV: the ratio between the standard deviation and the absolute value of the mean of the estimations provided by the subject under test), and which typically get better with experience.

   \begin{gather}
     a=b \label{one} \\
     c=d \label{two} \\
     e=f \label{three}
   \end{gather}
   \eqref{one} \eqref{two} \eqref{three}
